Feasibility Analysis of In-Band Coexistence in Dense LEO Satellite Communication Systems

This work provides a rigorous methodology for assessing the feasibility of spectrum sharing between large low-earth orbit (LEO) satellite constellations. For concreteness, we focus on the existing Starlink system and the soon-to-be-launched Kuiper system, which is prohibited from inflicting excessive interference onto the incumbent Starlink ground users. We carefully model and study the potential downlink interference between the two systems and investigate how strategic satellite selection may be used by Kuiper to serve its ground users while also protecting Starlink ground users. We then extend this notion of satellite selection to the case where Kuiper has limited knowledge of Starlink's serving satellite. Our findings reveal that there is always the potential for very high and extremely low interference, depending on which Starlink and Kuiper satellites are being used to serve their users. Consequently, we show that Kuiper can protect Starlink ground users with high probability, by strategically selecting which of its satellites are used to serve its ground users. Simultaneously, Kuiper is capable of delivering near-maximal downlink SINR to its own ground users. This highlights a feasible route to the coexistence of two dense LEO satellite systems, even in scenarios where one system has limited knowledge of the other's serving satellites.

==> DigComm_notation.tex <==
%\def\SNR{\mathrm{SNR}}
%\def\SINR{\mathrm{SINR}}
%\def\SIR{\mathrm{SIR}}
%\def\MMSE   {\mbox{\scriptsize \sf MMSE}}
%\def\sir {\mbox{\scriptsize\sf SIR}}
%\def\snr {\mbox{\scriptsize\sf SNR}}
%\def\sinr {\mbox{\scriptsize\sf SINR}}

\usepackage{xspace}

% \newcommand{\numbeams}{\ensuremath{N_{\mathrm{B}}}\xspace}

\def\sinc{\mbox{\textrm sinc}}

\def\Es{\mathcal{E}_s}
\def\Eb{\mathcal{E}_b}
\def\E{\mathbb{E}}
\def\dd{\mathrm{d}}

\newcommand{\ea}{\stackrel{(\text{a})}{=}}
\newcommand{\eb}{\stackrel{(\text{b})}{=}}
\newcommand{\ec}{\stackrel{(\text{c})}{=}}
\newcommand{\ed}{\stackrel{(\text{d})}{=}}
\newcommand{\ee}{\stackrel{(\text{e})}{=}}
\newcommand{\ef}{\stackrel{(\text{f})}{=}}
\newcommand{\eg}{\stackrel{(\text{g})}{=}}
\newcommand{\eh}{\stackrel{(\text{h})}{=}}
\newcommand{\ei}{\stackrel{(\text{i})}{=}}

%\newcommand*\diff{\mathop{}\!\mathrm{d}}

% Bold lowercase
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}


% Bold capital letters
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

==> sec-motivation.txt.tex <==
\begin{flushleft}
	
\end{flushleft}\section{Motivation and Scope} \label{sec:motivation}







==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

==> sec-preliminary.tex <==
\section{Preliminary Background on IPC} \label{sec:preliminary}
%The throughput degradation methodology as the IPC in real systems looks reasonable in several aspects.
%The purpose of imposing interference protection mechanisms on later-round systems is not just to limit the amount of energy leakages on earlier-round systems. 
%Instead, more importantly, earlier-round systems should still be able to achieve their target throughput, packet error rates, and spectral efficiency based on their actual implementation, even in the presence of interference while sharing the spectrum with later-round systems.  
%Considering advances in digital signal processing and receiver implementations, there are ways to avoid interference from other systems using, for example, advanced beamforming or antenna technologies. The FCC notices that modern systems can tolerate a certain level of interference, and communication can be successful even in heavy interference using lower modulation and coding schemes with repetition. 


Though FCC decided to adopt the throughput degradation methodology as the IPC, it is challenging to directly use the methodology as the IPC for research purposes in academia. Information on actual implementations of NGSO satellite systems, including adaptive modulation and coding schemes, frame structures, resource assignments, and retransmission mechanisms to measure the percentage degradation, is barely publicly available. 
Instead, we can use alternative measures as the IPC, such as the capacity degradation, \gsinr degradation, or \ginr limit, which are related to each other and can infer the throughput degradation to some extent. 


% IPC single entry vs aggregated entry
From the literature, IPC is generally defined in terms of carrier-to-interference ration (CIR) (equivalent to \gsnr) or \ginr \cite{} often specified with a condition of the long-term interference level not exceeding for more than a certain portion, for example $20\%$ of the time \cite{itu fixed satellite}. 
 IPC based on \ginr threshold often takes the value of $-6$ to $-10$ dB as a maximum \ginr, which can be inter-changeably defined using \gsnr as a $1$ dB drop in \gsnr is considered to be equivalent to $-6$ dB of \ginr \cite{1dbsnr}.


Geo-stationary orbit (GSO) systems have been incumbent over NGSO systems in the frequency spectrum that NGSO systems to share. 
ITU defines a coordination trigger to determine if coordination between two GSO and NGSO systems is required to prevent unacceptable mutual interference. The coordination trigger is defined in terms of the percentage increase in system noise temperature of a receiver of either system. 
The trigger level for determining if coordination action is required is 
 \begin{align}
 	\Delta \mathrm{T/T} \geq 6 \%, \label{eq:deltat}
 \end{align}
where $\mathrm{T}$ is a receiver noise temperature, and $\Delta\mathrm{T}$ is the increase in system noise temperature due to interfering signals. Rewriting \eqref{eq:deltat}, we have a trigger level in terms of \ginr 
\begin{align}
	\Delta \mathrm{T/T} = \minr  \geq 0.06% \,\, \todB{\minr} =-12.2.
\end{align}
using ${N} = k\cdot \mathrm{T} \cdot \mathrm{B}$ and $\mathrm{I} = k\cdot \Delta \mathrm{T} \cdot \mathrm{B}$ where $k$ is the Boltzmann's constant, and $\mathrm{B}$ is the bandwidth, and thus we have the trigger level as $\todB{\minr} \geq -12.2$. 




%\begin{figure*}[t]
%	\centering
%	\subfloat[\ginr impact on \gsinr.
%	]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{coex_fig/inr_vs_sinr}
%		\label{fig:inr-vs-sinr}}  
%	\hfill
%%		\subfloat[\ginr impact on normalized capacity
%%	]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{coex_fig/inr_vs_capacity}
%%		\label{fig:inr-vs-capacity}} \\
%	\subfloat[\ginr impact on normalized capacity
%	]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{coex_fig/inr_vs_norm_capacity}
%		\label{fig:inr-vs-capacity}} 
%	\caption{\ginr}
%	\label{fig:inr-impact-on-performance}
%\end{figure*}


